Solving Projected Model Counting by Utilizing Treewidth and its Limits

In this paper, we introduce a novel algorithm to solve projected model counting (PMC). PMC asks to count solutions of a Boolean formula with respect to a given set of projection variables, where multiple solutions that are identical when restricted to the projection variables count as only one solution. Inspired by the observation that the so-called "treewidth" is one of the most prominent structural parameters, our algorithm utilizes small treewidth of the primal graph of the input instance. More precisely, it runs in time O(2^2k+4n2) where k is the treewidth and n is the input size of the instance. In other words, we obtain that the problem PMC is fixed-parameter tractable when parameterized by treewidth. Further, we take the exponential time hypothesis (ETH) into consideration and establish lower bounds of bounded treewidth algorithms for PMC, yielding asymptotically tight runtime bounds of our algorithm. While the algorithm above serves as a first theoretical upper bound and although it might be quite appealing for small values of k, unsurprisingly a naive implementation adhering to this runtime bound suffers already from instances of relatively small width. Therefore, we turn our attention to several measures in order to resolve this issue towards exploiting treewidth in practice: We present a technique called nested dynamic programming, where different levels of abstractions of the primal graph are used to (recursively) compute and refine tree decompositions of a given instance. Finally, we provide a nested dynamic programming algorithm and an implementation that relies on database technology for PMC and a prominent special case of PMC, namely model counting (#Sat). Experiments indicate that the advancements are promising, allowing us to solve instances of treewidth upper bounds beyond 200.

==> algorithms/dpcountingfirst.tex <==

%\renewcommand{\tab}{Tab}
%\renewcommand{\AlgW}{\ensuremath{\mathtt{W}}}%
%\renewcommand{\AlgC}{\ensuremath{\mathtt{C}}}%

%\dpa_{\INCSAT}$,
%$\dpa_{\INCCOUNTERSAT}$ and $\cw_{\INCSAT, \INCCOUNTERSAT}$

\begin{algorithm}[H]
  % \KwData{Transition algorithm $\AlgA$, Program $\prog$ and
  % TD~$\TTT$ of graph of $\prog$ according to $\AlgA$.}%
  \KwData{
    % Table algorithms $\INCSAT$ and
    % $\INCCOUNTERSAT$, 
    Nice TD~$\TTT=(T,\chi)$ with
    $T=(N,\cdot,n)$ of a graph~$S(\prog)$,
    mapping $\ATab{\AlgW}[\cdot]$, and projection~$\cdot{\mid_t}$. %$\ATab{{\AlgW}}$,
    %$\ATab{\AlgC}[\cdot]$. %$\ATab{{\AlgC}}$.
    %
  }%
  \KwResult{$\ATab{\AlgC}$: maps node~$t\in
    T$ to some table of pairs~$\langle \tab{}, c\rangle$
    where~$c$ is an upper bound of the (combined) projected model count of $\tab{} \subseteq \ATabs{\AlgW}{t}$. } %
  %\tcc*[h]{For Abbreviations see
   % Footnote~\ref{foot:crossproduct}.\hspace{-0.05em}}
  
  $\Tab{}_t \eqdef \SB \ATab{\AlgC}[t'] \SM t' \text{ is a child of $t$ in
      $T$}\SE$\vspace{-0.05em} %
  
  \tcc*[h]{Get for a node~$t$ tables of (preceding) combined child rows (CCR)\vspace{-0.05em}}
    \vspace{-0.1em}$\label{algo3:ccr}\text{CCR}_t \eqdef \hat{\Pi}_{\tab{}' \in \Tab{}_t}\tab{}'$% i \in \{1, \dots, |\Tab{}|\}}\Tab{}[t']$
      %{t'\text{is a children of } t} \ATabs{\AlgW, \AlgC}{t'}$ %\ATabs{\AlgW}{t'}$%
\tcc*[f]{\hspace{-0.05em}Abbreviations below.\hspace{-0.05em}}
	  
    \tcc*[h]{Get for a row~$\vec \tabval$ its combined child rows (origins)} %
    $\label{algo3:orig}\orig_t(\vec \tabval) \eqdef %
    \SB S %
    \SM S \in \text{CCR}_t, \vec u \in \tab{}, \tab{} =
    {\AlgW}(t,\chi(t),\prog_t,\atto,S) %
    \SE$
      
    %\tcc*[h]{Get for a table~$S$ of combined child rows its successors (evolution)
%	%Find corresp. rows in parent table for set of counter or
%     % witness tables
%	 }\; $\label{algo3:evol}\evol_t(S) \eqdef %
%    \SB \vec \tabval \SM %
%    \vec \tabval \in \tab{}, %
%    \tab{} = {\AlgC}(t,\chi(t),\prog_t,\atto, \tab{}'), \tab{}'\in
%    S%
%    \SE$\vspace{0.3em}

    $bucketOf_t(\tab{}) \eqdef \{\vec\tabval_{\mid{_t}} \mid \vec\tabval\in \tab{}\}$

    $\tab{} =_{t} \tab{}' \eqdef bucketOf_t(\tab{}) = bucketOf_t(\tab{}')$

    $buckets_t \eqdef \{\tab{} \mid \tab{} \subseteq \ATabs{\AlgW}{t}, \not\exists \tab{}' \supsetneq \tab{}\ s.t.\ \tab{} =_{t} \tab{}', \card{bucketOf_t(\tab{})} = 1  \} $

    %$subbuckets_t \eqdef \{\tab{}' \mid \tab{}' \subseteq \tab{}, \tab{} \in buckets_t\}$

    %$cnt_t(S) \eqdef \Sigma_{c: \vec\tabval = \langle w, c \rangle, w \in S, \vec\tabval \in \ATabs{\AlgC}{t}} c$
    $cnt_t(S) \eqdef c \text{ iff } \vec\tabval = \langle w, c \rangle, w \in S, \vec\tabval \in \ATabs{\AlgC}{t}; 0 \text{ otherwise}$
    
    $ProjOverCnt_t(\tab{}) \eqdef $ %computedcnt_{child of t}(bucket_{child of t}(\tabval))$
    $\Pi_{t': t' \text{ is a child of } t \text{ in } T}\Sigma_{S \mid S \in buckets_{t'}, S \cap [\bigcup_{\vec\tabval\in\tab{}}\orig_t(\vec\tabval)] \neq \emptyset} cnt_{t'}(S) $

  \For{\label{algo3:for}\text{\normalfont iterate}
    $t$ in \text{\normalfont post-order}(T,n)}{\vspace{-0.05em}%
    % 
    % $\ATab{{\INCSAT}} \eqdef \dpa_\INCSAT(\cal
    % T)$ \text{\qquad $\dots$for any
    %   $\AlgA\in\{\INCSAT, \INCCOUNTERSAT\}$}\;
    %   %
	%

   \tcc*[h]{Assign for each leaf node the counter to~$1$}

   \uIf{$\type(t) = \leaf$}{%
     $\ATabs{\AlgC}{t} \leftarrow  \{\langle \tab{}, 1 \rangle \mid \tab{} \in buckets_t\}$
 	%\EndIIf 
   }%
   \uElse {%
		 $\ATabs{\AlgC}{t} \leftarrow \{\langle \tab{},ProjOverCnt_t(\tab{})\rangle \mid \tab{} \in buckets_t\}$
   }
    \vspace{-0.5em} }%
  \Return{$\ATabs{\AlgC}{\cdot}$}
\vspace{-0.15em}
  \caption{Algorithm
    $\ocw_{{\AlgW}}({\cal T}, \ATab{\AlgW}, \cdot{\mid_t})$ for
    overcounting the number of projected witnesses.}
\label{fig:algocount1}
%\input{flowchart}
\end{algorithm}


%\renewcommand{\tab}{\ensuremath{\tau}}

%\vspace{-1.5em}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "iclp2017"
%%% End:


==> algorithms/nextsol.tex <==
\begin{algorithm}[H]
  %\KwData{Transition algorithm ${\cal A}$, Program $\prog$ and TD~$\TTT$ of graph of $\prog$ according to ${\cal A}$.}%
  \KwData{TD~$\TTT=(T,\cdot)$ with
    $T=(N,\cdot,n)$, solution tuples~${\cal S}$, table~$\ATabs{\AlgC}{\cdot}$, total ordering~$\prec$ of $\corig_\cdot(\cdot)$.}% and $\Tabs{$\cdot$}$ obtained by preceding call to~$\dpa$.}%
  %\KwResult{Tables$:N \rightarrow 2^{\at(\prog)}$, mapping TD nodes to computed tables. } %
  \KwResult{The next solution tuples of~${\cal S}$ using~$\prec$. } %
  %\lForAll{$t \in N$}{%
  %  $\Tabs{t} \eqdef \text{undef}$%
  %}%
  %$o \eqdef $ post-order($T$)\;%
  %$\Tabs{$\cdot$} \lassign \vwe_{{\AlgW}}({\cal T}, \ATab{\AlgW}, \cdot{\mid_t})$
  
  \For{\text{\normalfont iterate} $t$ in \text{\normalfont post-order}(T,n)}{\vspace{-0.05em}%
    %$t \eqdef \text{next-node}(o)$\;%
    %$\att \eqdef \text{rules-below}({\cal T})$\;%
    %$\prog_t \eqdef \text{bag-rules}_{\cal A}(\prog,\chi(t))$\;%
    %$A_t \eqdef \text{bag-atoms}_{\cal A}(\prog,t,\TTT)$\;%
    $\Tab{} \eqdef \SB \ATabs{\AlgC}{t'} \SM t' \text{ is a child of $t$ in $T$}\SE$\vspace{-0.05em} %
	
	${\hat t} \eqdef \text{\normalfont parent of } t$
	
	${\cal S}[t] \lassign \text{\normalfont direct successor } s' \succ {\cal S}[{t}] \text{ in } \corig_{{\hat t}}({\cal S}[{\hat t}])$
	
	\If{${\cal S}[t]$ defined}{
		\For{\text{\normalfont iterate} $t'$ in \text{\normalfont \Tab{}}}{
			\For{\text{\normalfont iterate} $t''$ in \text{\normalfont pre-order}(T,t')}{\vspace{-0.05em}%
				${\hat t''} \eqdef \text{\normalfont parent of } t''$
				
				${\cal S}[t''] \lassign$ \text{\normalfont $\prec$-smallest element in $\corig_{{\hat t''}}({\cal S}[{\hat t''}])$} 
			\vspace{-0.3em}}
		\vspace{-0.3em}}
		\Return{${\cal S}$}
	\vspace{-0.3em}}
    \vspace{-0.3em} }\vspace{-0.1em}%
    \Return{undefined}
  \caption{Algorithm ${\nxt}_{\prec}({\cal T}, {\cal S}, \ATabs{\AlgC}{\cdot})$ for computing the $\prec$-next projected model.}
\label{fig:dpnext}
\end{algorithm}
%\vspace{-1.5em}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dl_dp"
%%% End:


==> algorithms/projmodelenum.tex <==

%\renewcommand{\tab}{Tab}
%\renewcommand{\AlgW}{\ensuremath{\mathtt{W}}}%
%\renewcommand{\AlgC}{\ensuremath{\mathtt{C}}}%

%\dpa_{\INCSAT}$,
%$\dpa_{\INCCOUNTERSAT}$ and $\cw_{\INCSAT, \INCCOUNTERSAT}$

\begin{algorithm}[H]
  % \KwData{Transition algorithm $\AlgA$, Program $\prog$ and
  % TD~$\TTT$ of graph of $\prog$ according to $\AlgA$.}%
  \KwData{
    % Table algorithms $\INCSAT$ and
    % $\INCCOUNTERSAT$, 
    Nice TD~$\TTT=(T,\chi)$ with
    $T=(N,\cdot,n)$ of a graph~$S(\prog)$,
    mapping $\ATab{\AlgW}[\cdot]$, and projection~$\cdot{\mid_t}$. %$\ATab{{\AlgW}}$,
    %$\ATab{\AlgC}[\cdot]$. %$\ATab{{\AlgC}}$.
    %
  }%
  \KwResult{$\ATab{\AlgC}$: maps node~$t\in
    T$ to some table of pairs~$\langle \tab{}\rangle$
    where $\tab{} \subseteq \ATabs{\AlgW}{t}; \corig_t(\tab{})$: gives for set~$\tab{}$ of tuples in node~$t$ its set of origins for projected enumeration. } %
  %\tcc*[h]{For Abbreviations see
   % Footnote~\ref{foot:crossproduct}.\hspace{-0.05em}}
  
  $\Tab{}_t \eqdef \SB \ATab{\AlgC}[t'] \SM t' \text{ is a child of $t$ in
      $T$}\SE$\vspace{-0.05em} %
  
  \tcc*[h]{Get for a node~$t$ tables of (preceding) combined child rows (CCR)\vspace{-0.05em}}
    \vspace{-0.1em}$\label{algo3:ccr}\text{CCR}_t \eqdef \hat{\Pi}_{\tab{}' \in \Tab{}_t}\tab{}'$% i \in \{1, \dots, |\Tab{}|\}}\Tab{}[t']$
      %{t'\text{is a children of } t} \ATabs{\AlgW, \AlgC}{t'}$ %\ATabs{\AlgW}{t'}$%
\tcc*[f]{\hspace{-0.05em}Abbreviations see below.\hspace{-0.05em}}
	  
    \tcc*[h]{Get for a row~$\vec \tabval$ its combined child rows (origins)} %
    $\label{algo3:orig}\orig_t(\vec \tabval) \eqdef %
    \SB S %
    \SM S \in \text{CCR}_t, \vec u \in \tab{}, \tab{} =
    {\AlgW}(t,\chi(t),\prog_t,\atto,S) %
    \SE$
      
    %\tcc*[h]{Get for a table~$S$ of combined child rows its successors (evolution)
%	%Find corresp. rows in parent table for set of counter or
%     % witness tables
%	 }\; $\label{algo3:evol}\evol_t(S) \eqdef %
%    \SB \vec \tabval \SM %
%    \vec \tabval \in \tab{}, %
%    \tab{} = {\AlgC}(t,\chi(t),\prog_t,\atto, \tab{}'), \tab{}'\in
%    S%
%    \SE$\vspace{0.3em}

    $bucketOf_t(\tab{}) \eqdef \{\vec\tabval_{\mid{_t}} \mid \vec\tabval\in \tab{}\}$

    $\tab{} =_{t} \tab{}' \eqdef bucketOf_t(\tab{}) = bucketOf_t(\tab{}')$

    $buckets_t \eqdef \{\tab{} \mid \tab{} \subseteq \ATabs{\AlgW}{t}, \not\exists \tab{}' \supsetneq \tab{}\ s.t.\ \tab{} =_{t} \tab{}', \card{bucketOf_t(\tab{})} = 1  \} $

    $subbuckets_t \eqdef \{\tab{}' \mid \tab{}' \subseteq \tab{}, \tab{} \in buckets_t\}$
   
    $origIn_t(\tab{}, t') \eqdef S \text{ where } S \subseteq \bigcup_{\vec\tabval \in \tab{}}\orig_t(\vec\tabval), S \neq \emptyset, S \subseteq \ATabs{\AlgC}{t'}, \not\exists S' \supsetneq S: S' \subseteq \ATabs{\AlgC}{t'}$

    $ProjOrigins_t(\tab{}) \eqdef $ %computedcnt_{child of t}(bucket_{child of t}(\tabval))$
    ${\hat\Pi}_{t': t' \text{ is a child of } t \text{ in } T}\{origIn_t(\tab{}, t')\}$ %S \mid S \subseteq \bigcup_{\vec\tabval \in \tab{}}\orig_t(\vec\tabval), S \neq \emptyset, S \subseteq \ATabs{\AlgC}{t'}\}$

  \For{\label{algo3:for}\text{\normalfont iterate}
    $t$ in \text{\normalfont post-order}(T,n)}{\vspace{-0.05em}%
    % 
    % $\ATab{{\INCSAT}} \eqdef \dpa_\INCSAT(\cal
    % T)$ \text{\qquad $\dots$for any
    %   $\AlgA\in\{\INCSAT, \INCCOUNTERSAT\}$}\;
    %   %
	%

   %\tcc*[h]{Assign for each leaf node the counter for ALL the subsets (also for the set itself) of a bucket to~$1$}

   $\ATabs{\AlgC}{t} \leftarrow  \{\langle \tab{} \rangle \mid \tab{} \in subbuckets_t\}$
   
   \uIf{$\type(t) = \leaf$}{%
     $\corig_t(\tab{}) \leftarrow \{\emptyset\}$ \qquad\qquad\qquad\qquad for $\tab{} \in subbuckets_t$
 	%\EndIIf 
   }%
   \uElse {%
     %$\ATabs{\AlgC}{t} \leftarrow \{\langle \tab{} \rangle \mid \tab{} \in subbuckets_t\}$ % \ATabs{\AlgW}{t}\}$
     $\corig_t(\tab{}) \leftarrow ProjOrigins_t({\tab{}})$ \qquad for $\tab{} \in subbuckets_t$
   }
   %\tcc*[h]{For computing the costs of one row, we might as well find among all the extension pointers the maximum subset of each bucket that is present in that way}
    \vspace{-0.5em} }\vspace{-0.00em}%
  \Return{$\ATabs{\AlgC}{\cdot}, \corig_{\cdot}(\cdot)$
  }\vspace{-0.2em}
  \caption{Algorithm
    $\cwe_{{\AlgW}}({\cal T}, \ATab{\AlgW}, \cdot{\mid_t})$ for
    preparing enumeration of projected witnesses.}
\label{fig:dpontdenum}
%\input{flowchart}
\end{algorithm}


%\renewcommand{\tab}{\ensuremath{\tau}}

%\vspace{-1.5em}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "iclp2017"
%%% End:


==> algorithms/satovercounting.tex <==

%\renewcommand{\tab}{Tab}
%\renewcommand{\PRIM}{\ensuremath{\mathtt{W}}}%
%\renewcommand{\PROJ}{\ensuremath{\mathtt{C}}}%

%\dpa_{\INCSAT}$,
%$\dpa_{\INCCOUNTERSAT}$ and $\cw_{\INCSAT, \INCCOUNTERSAT}$

\begin{algorithm}[H]
  % \KwData{Transition algorithm $\AlgA$, Program $\prog$ and
  % TD~$\TTT$ of graph of $\prog$ according to $\AlgA$.}%
  \KwData{
    % Table algorithms $\INCSAT$ and
    % $\INCCOUNTERSAT$, 
    Nice TD~$\TTT=(T,\chi)$ with
    $T=(N,\cdot,n)$ of a graph~$P(\prog)$,
    mapping $\ATab{\PRIM}[\cdot]$, and projection~$\cdot{\mid_t}$. %$\ATab{{\PRIM}}$,
    %$\ATab{\PROJ}[\cdot]$. %$\ATab{{\PROJ}}$.
    %
  }%
  \KwResult{$\ATab{\PROJ}$: maps node~$t\in
    T$ to some table of pairs~$\langle \tab{}, c\rangle$
    where~$c$ is an upper bound of the (combined) projected model count of $\tab{} \subseteq \ATabs{\PRIM}{t}$. } %
  %\tcc*[h]{For Abbreviations see
   % Footnote~\ref{foot:crossproduct}.\hspace{-0.05em}}
  
  $\Tab{}_t \eqdef \SB \ATab{\PROJ}[t'] \SM t' \text{ is a child of $t$ in
      $T$}\SE$\vspace{-0.05em} %
  
  \tcc*[h]{Get for a node~$t$ tables of (preceding) combined child rows (CCR)\vspace{-0.05em}}
    \vspace{-0.1em}$\label{algo3:ccr}\text{CCR}_t \eqdef \hat{\Pi}_{\tab{}' \in \Tab{}_t}\tab{}'$% i \in \{1, \dots, |\Tab{}|\}}\Tab{}[t']$
      %{t'\text{is a children of } t} \ATabs{\PRIM, \PROJ}{t'}$ %\ATabs{\PRIM}{t'}$%
%\tcc*[f]{\hspace{-0.05em}Abbreviations below.\hspace{-0.05em}}
	  
    \tcc*[h]{Get for a row~$\vec \tabval$ its combined child rows (origins)} %
    $\label{algo3:orig}\orig_t(\vec \tabval) \eqdef %
    \SB S %
    \SM S \in \text{CCR}_t, \vec u \in \tab{}, \tab{} =
    {\PRIM}(t,\chi(t),\prog_t,S) %
    \SE$
      
    %\tcc*[h]{Get for a table~$S$ of combined child rows its successors (evolution)
%	%Find corresp. rows in parent table for set of counter or
%     % witness tables
%	 }\; $\label{algo3:evol}\evol_t(S) \eqdef %
%    \SB \vec \tabval \SM %
%    \vec \tabval \in \tab{}, %
%    \tab{} = {\PROJ}(t,\chi(t),\prog_t,\atto, \tab{}'), \tab{}'\in
%    S%
%    \SE$\vspace{0.3em}

    $bucketOf_t(\tab{}) \eqdef \{\vec\tabval_{\mid{_t}} \mid \vec\tabval\in \tab{}\}$

    $\tab{} =_{t} \tab{}' \eqdef bucketOf_t(\tab{}) = bucketOf_t(\tab{}')$

    $buckets_t \eqdef \{\tab{} \mid \tab{} \subseteq \ATabs{\PRIM}{t}, \not\exists \tab{}' \supsetneq \tab{}\ s.t.\ \tab{} =_{t} \tab{}', \card{bucketOf_t(\tab{})} = 1  \} $

    %$subbuckets_t \eqdef \{\tab{}' \mid \tab{}' \subseteq \tab{}, \tab{} \in buckets_t\}$

    %$cnt_t(S) \eqdef \Sigma_{c: \vec\tabval = \langle w, c \rangle, w \in S, \vec\tabval \in \ATabs{\PROJ}{t}} c$
    $cnt_t(S) \eqdef c \text{ iff } \vec\tabval = \langle w, c \rangle, w \in S, \vec\tabval \in \ATabs{\PROJ}{t}; 0 \text{ otherwise}$
    
    $ProjOverCnt_t(\tab{}) \eqdef $ %computedcnt_{child of t}(bucket_{child of t}(\tabval))$
    $\Pi_{t': t' \text{ is a child of } t \text{ in } T}\Sigma_{S \mid S \in buckets_{t'}, S \cap [\bigcup_{\vec\tabval\in\tab{}}\orig_t(\vec\tabval)] \neq \emptyset} cnt_{t'}(S) $

  \For{\text{\normalfont iterate}
    $t$ in \text{\normalfont post-order}(T,n)}{\vspace{-0.05em}%
    % 
    % $\ATab{{\INCSAT}} \eqdef \dpa_\INCSAT(\cal
    % T)$ \text{\qquad $\dots$for any
    %   $\AlgA\in\{\INCSAT, \INCCOUNTERSAT\}$}\;
    %   %
	%

   \tcc*[h]{Assign for each leaf node the counter to~$1$}

   \uIf{$\type(t) = \leaf$}{%
     $\ATabs{\PROJ}{t} \leftarrow  \{\langle \tab{}, 1 \rangle \mid \tab{} \in buckets_t\}$
 	%\EndIIf 
   }%
   \uElse {%
		 $\ATabs{\PROJ}{t} \leftarrow \{\langle \tab{},ProjOverCnt_t(\tab{})\rangle \mid \tab{} \in buckets_t\}$
   }
    \vspace{-0.5em} }%
  \Return{$\ATabs{\PROJ}{\cdot}$}
\vspace{-0.15em}
  \caption{Algorithm
    $\ocw_{\PRIM}({\cal T}, \ATab{\PRIM}, \cdot{\mid_t})$ for
    overcounting the number of projected witnesses.}
\label{fig:algocount1}
%\input{flowchart}
\end{algorithm}


%\renewcommand{\tab}{\ensuremath{\tau}}

%\vspace{-1.5em}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "iclp2017"
%%% End:


==> figures/style.tex <==
\usetikzlibrary{positioning}
\usetikzlibrary{shapes,arrows}
\tikzstyle{arg}=[draw, thick, circle]

\colorlet{afnodecolor}{green!20!blue!10}
\colorlet{tdnodecolor}{green!20!blue!10}
\colorlet{subfwnodecolor}{black!2}
\colorlet{subfwafinactivenodecolor}{white}
\colorlet{vertexTopColor}{white}
%\colorlet{vertexBottomColor}{blue!20!black!15}
\colorlet{vertexBottomColor}{black!10}

\tikzstyle{afnode} = [draw,thick,shape=circle,minimum size=8mm,font=\normalsize,fill=afnodecolor]
\tikzstyle{afedge} = [->,draw,thick]
\tikzstyle{tdnode} = [draw,rounded corners,top color=vertexTopColor,bottom color=vertexBottomColor,minimum size=1.5em]
\tikzstyle{stdnode} = [tdnode, font=\scriptsize]
\tikzstyle{stdnodecompact} = [stdnode, inner sep = 1.5pt, outer sep = 0.1pt]
\tikzstyle{stdnodetable} = [stdnode, inner sep = 1.5pt, outer sep = 0]
\tikzstyle{stdnodenum} = [minimum size=1.5em, font=\scriptsize]
\tikzstyle{tdedge} = [-,draw,thick]
\tikzstyle{tdlabel} = [draw=none, rectangle, fill=none, inner sep=0pt, font=\scriptsize]
\tikzstyle{subfwnode} = [draw,thick,shape=rectangle,thin,rounded corners,minimum size=9mm,fill=subfwnodecolor,label distance=-2.5mm]
\tikzstyle{subfwafactivenode} = [draw,thick,shape=circle,minimum size=6mm,inner sep = 0pt,font=\scriptsize,fill=afnodecolor]
\tikzstyle{subfwafinactivenode} = [draw,thick,shape=circle,minimum size=6mm,inner sep = 0pt,font=\scriptsize,fill=white,dotted]
\tikzstyle{subfwafinactiveedge} = [->,draw,thick,dotted]

\tikzstyle{itemTree}=[level distance=2em,sibling distance=4ex,child anchor=west,grow'=right,right,align=left,every node/.style={draw,dashed,draw opacity=0.2,font=\footnotesize}]
\tikzstyle{itemTreeRoot}=[solid,inner sep=2]
\tikzstyle{orNode}=[label=left:$\lor$]
\tikzstyle{andNode}=[label=left:$\land$]
\tikzstyle{acceptNode}=[label=right:$\top$]
\tikzstyle{rejectNode}=[label=right:$\bot$]


==> figures/tables.tex <==
\begin{tikzpicture}[node distance=2mm]
%\tikzset{every node/.style=tdnode}
\tikzset{every path/.style=thick}

\scalebox{0.94}{
\node (rt) [stdnodecompact, label={[tdlabel, xshift=0.2em,yshift=-0.1em]right:$t_{5}$}]{$\{a'_1, a'_2, a'_3\}$};
\node (rt0) [stdnodecompact, below=of rt,label={[tdlabel, xshift=-1.75em,yshift=-0.0em]above left:$t_{4}$}]{$\{b_1, b_2, b_3, a'_1, a'_2, a'_3\}$};
\node (rt1) [stdnodecompact, below=of rt0,label={[tdlabel, xshift=0.2em,yshift=-0.1em]right:$t_{3}$}]{$\{b_1, b_2, b_3\}$};
\node (r2) [stdnodecompact, below=of rt1,label={[tdlabel, xshift=-1.75em,yshift=-0.0em]above left:${t_{2}}$}]{$\{a_1, a_2, a_3, b_1, b_2, b_3\}$};
\node (r3) [stdnodecompact, below=of r2,label={[tdlabel, xshift=0.2em,yshift=-0.1em]right:${t_{1}}$}]{$\{a_1, a_2, a_3\}$};

\node (r4) [below=of r3]{$\dots$};
\node (r0) [above=of rt]{$\dots$};
\node (td) [left=of r0,xshift=0.75em]{${\cal T\hspace{-0.4em}:}$};

\draw [dotted, ->] (r4) to (r3);
\draw [dotted, ->] (r3) to (r2);
\draw [dotted, ->] (r2) to (rt1);
\draw [dotted, ->] (rt1) to (rt0);
\draw [dotted, ->] (rt0) to (rt);
\draw [dotted, ->] (rt) to (r0);


%t1
\node (r3tab) [stdnodecompact,right=of r3,xshift=1.75em,yshift=-0.0em,label={[tdlabel, xshift=0em,  yshift=-0.75em]above left:$ \tab{1} $}] {\input{tables/r3tab}};
%t2
\node (r2tab) [stdnodecompact,right=of r3tab,xshift=0em,yshift=-0.0em,label={[tdlabel, xshift=-0.5em,  yshift=-0.85em]above left:$\tab{2}$}] {\input{tables/r2tab}};
%t3
\node (r1tab) [stdnodecompact,right=of r2tab,xshift=0em,yshift=-0.0em,label={[tdlabel,  yshift=0.1em]above right:$\tab{3}$}] {\input{tables/r1tab}};
%t4
\node (r4tab) [stdnodecompact,above=of r3tab,xshift=2.8em,yshift=-0.0em,label={[tdlabel, xshift=-1.5em, yshift=-0.85em]above left:$\tab{4}$}] {\input{tables/r4tab}};
%t5
\node (r5tab) [stdnodecompact,right=of r4tab,xshift=0em,yshift=-0.0em,label={[tdlabel, xshift=0.95em,  yshift=-0.85em]above right:$\tab{5}$}] {\input{tables/r5tab}};
}



%
%%t14
%\node (joinr) [stdnodecompact,right=of rt2,xshift=4.7em,yshift=-1.4em,label={[tdlabel,  yshift=-0.25em]below:$ $}] {\input{graph4_norm/tables_inc/r8_asp}};
%%%t16
%%\node (leaf2r) [stdnodecompact,above=of joinr,xshift=-0.35em,label={[tdlabel,  xshift=-0.5em,yshift=0.25em]above:$ $}] {\input{graph4_norm/tables_inc/r5_asp}};
%%t17
%
%\node (leaf1r) [stdnodecompact,right=of joinr,label={[tdlabel,  xshift=-0.5em,yshift=0.25em]above:$ $}] {\input{graph4_norm/tables_inc/r6_asp}};
%
%%t5
%\node (r14n) [stdnodetable,below=of joinr,xshift=-0.76em,label={[tdlabel, xshift=2em,yshift=+0.3em]above left:$ $}] {\input{graph4_norm/tables_inc/r14}};
%%t7
%\node (r14b) [stdnodecompact,right= of r14n,xshift=-0.05em, label={[tdlabel,  yshift=-0.25em]below:$ $}] {\input{graph4_norm/tables_inc/r14_asp}};
%%t3
%\node (leaf1) [stdnodetable,below =of r14n,xshift=-0.26em,label={[tdlabel, xshift=0em,yshift=+0.25em]above left:$ $}]{\input{graph4_norm/tables_inc/r5}};
%%t4
%\node (join) [stdnodetable,right=of leaf1, label={[tdlabel, xshift=2em,yshift=-0.25em]below left:$ $}] {\input{graph4_norm/tables_inc/r8}};
%
%\scalebox{0.95}{
%%t1
%\node (leaf0) [stdnode,left=of leaf1, xshift=0.5em,yshift=-2.35em] {\input{graph4_norm/tables_inc/leaf00}};
%}

 \end{tikzpicture}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dbai-tr-2016-101"
%%% End:


==> intersection.tex <==
\begin{tikzpicture}
	\draw[color=red,ultra thick,fill=yellow] plot[smooth, tension=.7] coordinates {(-4.5,0) (-6.5,-0.5) (-7,-2) (-6.5,-3.5) (-3.5,-5) (-2,-4) (-1.5,-2) (-2.5,0) (-4.5,0)};
	\draw[color=green,ultra thick,fill=yellow]  plot[smooth, tension=.7] coordinates {(-10.5,-6.5) (-13.5,-6) (-10.5,-3.5) (-5.5,-2) (-5,-3.5) (-6.5,-6) (-10.5,-6.5)};
	\draw[color=blue,ultra thick,fill=yellow]  plot[smooth, tension=.7] coordinates {(-4,-8.5) (-7.5,-6.5) (-13.5,-4) (-14.5,0.5) (-7,1) (-3.5,0) (-4.5,-4) (-7,-4.5) (-3.5,-7.5) (-4,-8.5)};
	

	\draw[color=red,ultra thick] plot[smooth, tension=.7] coordinates {(-4.5,0) (-6.5,-0.5) (-7,-2) (-6.5,-3.5) (-3.5,-5) (-2,-4) (-1.5,-2) (-2.5,0) (-4.5,0)};
	\draw[color=green,ultra thick]  plot[smooth, tension=.7] coordinates {(-10.5,-6.5) (-13.5,-6) (-10.5,-3.5) (-5.5,-2) (-5,-3.5) (-6.5,-6) (-10.5,-6.5)};
	\draw[color=blue,ultra thick]  plot[smooth, tension=.7] coordinates {(-4,-8.5) (-7.5,-6.5) (-13.5,-4) (-14.5,0.5) (-7,1) (-3.5,0) (-4.5,-4) (-7,-4.5) (-3.5,-7.5) (-4,-8.5)};
	
	
	\draw[color=black,ultra thick]  plot[smooth, tension=.7] coordinates {(-7,7) (-9.5,6) (-8.5,5.5) (-7.5,5) (-5,5.5) (-5,6.5) (-4,7) (-5,7.5) (-6.5,7.5) (-7,7)};

    
	\draw[ultra thick,->] (-7,6) -- (-9.5,-0.5);
	\draw[ultra thick,->] (-7.5,6) -- (-12,0); 
	\draw[ultra thick,->] (-6,6) -- (-4.5,-1.5);
	\draw[ultra thick,->] (-6.5,6) -- (-8,-4);

	
      \tikzstyle{gray_block} = [draw,outer sep=7,inner sep=7,minimum size=57,line width=1, very thick, draw=black!55, top color=white,bottom color=black!20]
    
	
\draw[gray_block]  (1,5.5) rectangle (10,2);
\draw[gray_block]  (1,1) rectangle (10,-7);

\draw[ball color=blue] (0,0) circle (.5);


      \makeatletter
      \pgfdeclareshape{document}{
      \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
      \inheritanchorborder[from=rectangle]
      \inheritanchor[from=rectangle]{center}
      \inheritanchor[from=rectangle]{north}
      \inheritanchor[from=rectangle]{south}
      \inheritanchor[from=rectangle]{west}
      \inheritanchor[from=rectangle]{east}
      % ... and possibly more
      \backgroundpath{% this is new
      % store lower right in xa/ya and upper right in xb/yb
      \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
      \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
      % compute corner of ``flipped page''
      \pgf@xc=\pgf@xb \advance\pgf@xc by-5pt % this should be a parameter
      \pgf@yc=\pgf@yb \advance\pgf@yc by-5pt
      % construct main path
      \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
      \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
      \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
      \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
      \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
      \pgfpathclose
      % add little corner
      \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
      \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
      \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
      \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
      }
      }
      \tikzstyle{message} = [shape=document, thick, draw=black, minimum width=2cm]
    
    \node at (0,0) [forbidden sign,line width=2ex,draw=red,fill=white] {Smoking};
    
    \tikzset{button/.style={
% First preaction: Fuzzy shadow
preaction={fill=black,path fading=circle with fuzzy edge 20 percent,
opacity=.5,transform canvas={xshift=1mm,yshift=-1mm}},
% Second preaction: Background pattern
preaction={pattern=#1,
path fading=circle with fuzzy edge 15 percent},
% Third preaction: Make background shiny
preaction={top color=white,
bottom color=black!50,
shading angle=45,
path fading=circle with fuzzy edge 15 percent,
opacity=0.2},
% Fourth preaction: Make edge especially shiny
preaction={path fading=fuzzy ring 15 percent,
top color=black!5,
bottom color=black!80,
shading angle=45},
inner sep=2ex
}, 
button/.default=horizontal lines light blue,
circle}
    
      \tikzstyle{bordered} = [draw,outer sep=0,inner sep=1,minimum size=10]
     
      
\end{tikzpicture}


